SynDe: Syndrome-guided Decoding of Raw Nanopore Reads

Nanopore sequencing technology remains highly error-prone, making efficient error correction essential in DNA-based data storage. Prior work addressed high error rates using convolutional codes with their decoder coupled with the basecaller, but such approaches only accommodate a limited number of code classes and incur significant decoding complexity. To overcome these limitations, we propose two algorithms: PrimerSeeker, which efficiently detects primer sequences in raw nanopore sequencing reads, and SynDe, a decoder that operates on the same raw reads and supports any linear error correction code with a low-complexity graphical representation. PrimerSeeker provides primer location estimates close to those of existing approaches while being better suited for real-time primer detection during sequencing. SynDe performs well with convolutional codes augmented with periodic markers, often approaching or exceeding the performance of existing algorithms with a lower time complexity. Remarkably, the confidence scores produced by SynDe reliably identify which of its outputs should be discarded.

==> resources/decoding-pipeline/syndrome-trellis-dna.tex <==
\begin{tikzpicture}[long dash/.style={dash pattern=on 10pt off 2pt}, short dash/.style={ dash pattern=on 3pt off 2.4pt}, ->,>=stealth]

    \tikzstyle{tiny dot}=[circle, fill, inner sep=0.5pt]
    \tikzstyle{syndrome node}=[circle, inner sep=4pt, fill=brown!15,font=\small]
    \newlength{\vsep}
    \newlength{\hsep}
    \setlength{\vsep}{1.3cm}%{0.35cm}
    \setlength{\hsep}{1.5cm}%{0.67cm}

    % ----- highlighting info, parity and termination stages in color
    % \foreach \j/\col in {-3/green, -2/green, 0/green, 1/green, -1/blue, 2/blue, 3/red, 4/red, 5/red}{
    %     \fill[fill=\col!20, opacity=0.4] ($(\j*\hsep, 0)$) rectangle ($(\j*\hsep + \hsep, -7*\vsep)$);
    % }

    % ---- drawing nodes in trellis -------
    % \foreach \i in {0,1,2,3}{
    %     \foreach \j in {-3,-2,-1,0,1,2,3,4,5,6,7}{
    %         \node[draw, syndrome node] (x\i\j) at ($(\j*\hsep, -\i*\vsep)$){};
    % }

    \foreach \j/\i/\synstate in {0/0/0, 
                                1/0/0, 1/1/160,
                                2/0/0, 2/1/80,
                                3/0/0, 3/1/80, 3/2/100, 3/3/52,
                                4/0/0, 4/1/16, 4/2/36, 4/3/52,
                                5/0/0, 5/1/56, 5/2/36, 5/3/28,
                                6/0/0, 6/1/24, 6/2/4, 6/3/28,
                                7/0/0, 7/1/24, 7/2/29, 7/3/5,
                                8/0/0, 8/1/20,
                                9/0/0, 9/1/60,
                                10/0/0}{
            \node[draw, syndrome node] (x\j\synstate) at ($(\j*\hsep, -\i*\vsep)$){\synstate};
    }
    
    % --------------------------------------------
    % 0 edges (straight)
    \foreach \ia/\syna/\ib/\synb in {2/0/3/0,3/0/4/0,4/0/5/0,5/0/6/0,6/0/7/0,7/0/8/0,
    2/80/3/80,3/52/4/52,4/36/5/36,5/28/6/28,6/24/7/24}{
        \draw[->, short dash] (x\ia\syna) -- (x\ib\synb);
    }      
    % edges curved
    \draw[->, solid] (x00.south) to [out=-90,in=180] (x1160.west);
    %\draw[->, solid] (x20.east) to [out=-5,in=180] (x325.west);
    \draw[->, solid] (x280.south) to [out=-90,in=180] (x352.west);    
    \draw[->, solid] (x380.east) to [out=0,in=180] (x436.west);
    %\draw[->, solid] (x325.east) to [out=0,in=180] (x416.west);
    %\draw[->, solid] (x556.east) to [out=-5,in=180] (x64.west);
    \draw[->, solid] (x536.east) to [out=-5,in=180] (x624.west);
    \draw[->, short dash] (x75.east) to [out=5,in=265] (x820.south);
    %\draw[->, solid] (x729.east) to [out=5,in=180] (x80.west);
    \draw[->, solid] (x960.east) to [out=5,in=265] (x100.south);
    
    % 1 edges  (straight)
    \foreach \ia/\syna/\ib/\synb in {1/160/2/80,4/16/5/56,4/52/5/28,6/28/7/5,7/24/8/20,8/20/9/60}{
        \draw[->, solid] (x\ia\syna) -- (x\ib\synb);
    }

    % ======= highlight codeword =========
    \draw[->, short dash, green!40!black] (x00) -- (x10);
    \draw[->, short dash, green!40!black] (x10) -- (x20);
    \draw[->, solid, green!40!black] (x20.east) to [out=-5,in=180] (x3100.west);
    \draw[->, solid, green!40!black] (x3100.east) to [out=0,in=180] (x416.west);
    \draw[->, solid, green!40!black] (x416) -- (x556);
    \draw[->, solid, green!40!black] (x556.east) to [out=-5,in=180] (x64.west);
    \draw[->, solid, green!40!black] (x64) -- (x729);
    \draw[->, solid, green!40!black] (x729.east) to [out=5,in=180] (x80.west);
    \draw[->, short dash, green!40!black] (x80) -- (x90);
    \draw[->, short dash, green!40!black] (x90) -- (x100);
    
    % \draw[->, solid, green] () -- ();
    % \draw[->, solid, green] () -- ();
    % \draw[->, solid, green] () -- ();
    % \draw[->, solid, green] () -- ();
    % \draw[->, short dash, green] () -- ();
    % \draw[->, short dash, green] () -- ();
    

\end{tikzpicture}

==> resources/primer_search_image.tex <==
\tikzset{
		child_beam/.style={
			draw=red,
			thick,
			ellipse,
			minimum width=1.2cm,
			minimum height=0.8cm,
			align=center
		},
		parent_beam/.style={
			draw=blue,
			thick,
			ellipse,
			minimum width=1.2cm,
			minimum height=0.8cm,
			align=center
		},
		child_edge/.style={
			->,
			>=stealth,
			thick,
			black
		},
		carry_edge/.style={
			dashed,
			gray,
			thick
		}
	}
	
	% Macros for drawing the objects
	\newcommand{\childbeam}[3]{\node[child_beam] (#1) at #2 {#3};}
	\newcommand{\parentbeam}[3]{\node[parent_beam] (#1) at #2 {#3};}
	\newcommand{\childedge}[4][]{\draw[child_edge] #2 -- #3 node[midway, above, font=\small] {#4} #1;}
	\newcommand{\childedgebelow}[4][]{\draw[child_edge] #2 -- #3 node[midway, below, font=\small] {#4} #1;}
	%\newcommand{\childedgeboth}[5][]{\draw[child_edge] #2 -- #3 node[midway, above, font=\small] {#4} node[midway, below, font=\small] {#5} #1;}
	\newcommand{\childedgeboth}[5][]{\draw[child_edge] #2 -- #3 node[midway, above, sloped, font=\footnotesize] {#4} node[midway, below, sloped, font=\footnotesize] {#5} #1;}
	\newcommand{\carryedge}[2]{\draw[carry_edge] #1 -- #2;}
	\begin{tikzpicture}[node distance=2.5cm and 2cm]
		\def\hsep{4.2cm}
		\def\vsep{8cm}
		
		% initial empty beams
		\parentbeam{start_a}{(0,0)}{start = a}
		\parentbeam{start_b}{(0,-\vsep)}{start = b}
		
		
		% first k-mer extensions
		\childbeam{s1_a_ca}{(\hsep,0)}{start = a\\CA}
		\childbeam{s1_b_ca}{(\hsep,-\vsep)}{start = b\\CA}
		
		\childedgeboth{(start_a)}{(s1_a_ca)}{$k$-mer CA}{at sample $x_a$}
		\childedgeboth{(start_b)}{(s1_b_ca)}{$k$-mer CA}{at sample $x_b$}
		
		
		% ============= level 1 ===================
		\parentbeam{s1_a_ca_parent}{($(s1_a_ca) + (\hsep,0)$)}{start = a\\CA}
		\parentbeam{s1_b_ca_parent}{($(s1_b_ca) + (\hsep,0)$)}{start = b\\CA} 
		
		\carryedge{(s1_a_ca)}{(s1_a_ca_parent)}
		\carryedge{(s1_b_ca)}{(s1_b_ca_parent)}
		
		\childbeam{s1_a_ca_dwell}{($(s1_a_ca_parent) + (\hsep,2cm)$)}{start = a\\CA}
		\childbeam{s1_a_ca_ext}{($(s1_a_ca_parent) + (\hsep,-2cm)$)}{start = a\\AC}
		
		\childbeam{s1_b_ca_dwell}{($(s1_b_ca_parent) + (\hsep,2cm)$)}{start = b\\CA}
		\childbeam{s1_b_ca_ext}{($(s1_b_ca_parent) + (\hsep,-2cm)$)}{start = b\\AC}
		
		\childedgeboth{(s1_a_ca_parent)}{(s1_a_ca_dwell)}{dwell at}{sample $x_{a+1}$}
		\childedgeboth{(s1_a_ca_parent)}{(s1_a_ca_ext)}{extend at}{sample $x_{a+1}$}
		
		\childedgeboth{(s1_b_ca_parent)}{(s1_b_ca_dwell)}{dwell at}{sample $x_{b+1}$}
		\childedgeboth{(s1_b_ca_parent)}{(s1_b_ca_ext)}{extend at}{sample $x_{b+1}$}
		
		% ============= level 2 ================
		\parentbeam{s2_a_ca}{($(s1_a_ca_dwell) + (\hsep,0)$)}{start = a\\CA}
		\parentbeam{s2_a_ac}{($(s1_a_ca_ext) + (\hsep,0)$)}{start = a\\AC} 
		\parentbeam{s2_b_ca}{($(s1_b_ca_dwell) + (\hsep,0)$)}{start = b\\CA}
		\parentbeam{s2_b_ac}{($(s1_b_ca_ext) + (\hsep,0)$)}{start = b\\AC} 
		
				
		\carryedge{(s1_a_ca_dwell)}{(s2_a_ca)}
		\carryedge{(s1_a_ca_ext) }{(s2_a_ac)}
		\carryedge{(s1_b_ca_dwell)}{(s2_b_ca)}
		\carryedge{(s1_b_ca_ext)}{(s2_b_ac)}
		
		% extend at level 2 (start=a, CA)
		\childbeam{s2_a_ca_dwell}{($(s2_a_ca) + (\hsep,1.1cm)$)}{start = a\\CA}
		\childbeam{s2_a_ca_ext}{($(s2_a_ca) + (\hsep,-1.1cm)$)}{start = a\\AC}
		\childedgeboth{(s2_a_ca)}{(s2_a_ca_dwell)}{dwell at}{sample $x_{a+2}$}
		\childedgeboth{(s2_a_ca)}{(s2_a_ca_ext)}{extend at}{sample $x_{a+2}$}
		
		% extend at level 2 (start=a, AC)
		\childbeam{s2_a_ac_dwell}{($(s2_a_ac) + (\hsep,1.1cm)$)}{start = a\\AC}
		\childbeam{s2_a_ac_ext}{($(s2_a_ac) + (\hsep,-1.1cm)$)}{start = a\\CG}
		\childedgeboth{(s2_a_ac)}{(s2_a_ac_dwell)}{dwell at}{sample $x_{a+2}$}
		\childedgeboth{(s2_a_ac)}{(s2_a_ac_ext)}{extend at}{sample $x_{a+2}$}
		
		% extend at level 2 (start=b, CA)
		\childbeam{s2_b_ca_dwell}{($(s2_b_ca) + (\hsep,1.1cm)$)}{start = b\\CA}
		\childbeam{s2_b_ca_ext}{($(s2_b_ca) + (\hsep,-1.1cm)$)}{start = b\\AC}
		\childedgeboth{(s2_b_ca)}{(s2_b_ca_dwell)}{dwell at}{sample $x_{b+2}$}
		\childedgeboth{(s2_b_ca)}{(s2_b_ca_ext)}{extend at}{sample $x_{b+2}$}
		
		% extend at level 2 (start=b, AC)
		\childbeam{s2_b_ac_dwell}{($(s2_b_ac) + (\hsep,1.1cm)$)}{start = b\\AC}
		\childbeam{s2_b_ac_ext}{($(s2_b_ac) + (\hsep,-1.1cm)$)}{start = b\\CG}
		\childedgeboth{(s2_b_ac)}{(s2_b_ac_dwell)}{dwell at}{sample $x_{b+2}$}
		\childedgeboth{(s2_b_ac)}{(s2_b_ac_ext)}{extend at}{sample $x_{b+2}$}
		
		% ======== level 3 =================
		\parentbeam{s3_a_ca}{($(s2_a_ca_dwell) + (\hsep,0)$)}{start = a\\CA}
		\parentbeam{s3_a_cg}{($(s2_a_ac_ext) + (\hsep,0)$)}{start = a\\CG}
		\carryedge{(s2_a_ca_dwell)}{(s3_a_ca)}
		\carryedge{(s2_a_ac_ext) }{(s3_a_cg)}
		
		\parentbeam{s3_b_ca}{($(s2_b_ca_dwell) + (\hsep,0)$)}{start = b\\CA}
		\parentbeam{s3_b_cg}{($(s2_b_ac_ext) + (\hsep,0)$)}{start = b\\CG}
		\carryedge{(s2_b_ca_dwell)}{(s3_b_ca)}
		\carryedge{(s2_b_ac_ext) }{(s3_b_cg)}
		
		% merged beams at level 3
		\parentbeam{s3_a_ac}{($(s2_a_ac_ext) + (\hsep,3.25cm)$)}{start = a\\AC}
		\parentbeam{s3_b_ac}{($(s2_b_ac_ext) + (\hsep,3.25cm)$)}{start = b\\AC}
		\carryedge{(s2_a_ca_ext)}{(s3_a_ac)}
		\carryedge{(s2_a_ac_dwell)}{(s3_a_ac)}
		\carryedge{(s2_b_ca_ext)}{(s3_b_ac)}
		\carryedge{(s2_b_ac_dwell)}{(s3_b_ac)}
		
		% edges to phantom nodes
		\foreach \cn in {s3_a_ca, s3_a_ac, s3_a_cg} {
			% \childedgeboth{(\cn)}{($(\cn) + (\hsep,0.8cm)$)}{dwell at}{sample $x_{a+3}$}
			% \childedgeboth{(\cn)}{($(\cn) + (\hsep,-0.8cm)$)}{extend at}{sample $x_{a+3}$}
            \childedgeboth{(\cn)}{($(\cn) + (\hsep,0.8cm)$)}{}{}
			\childedgeboth{(\cn)}{($(\cn) + (\hsep,-0.8cm)$)}{}{}
		}
		\foreach \cn in {s3_b_ca, s3_b_ac, s3_b_cg} {
			% \childedgeboth{(\cn)}{($(\cn) + (\hsep,0.8cm)$)}{dwell at}{sample $x_{b+3}$}
			% \childedgeboth{(\cn)}{($(\cn) + (\hsep,-0.8cm)$)}{extend at}{sample $x_{b+3}$}
            \childedgeboth{(\cn)}{($(\cn) + (\hsep,0.8cm)$)}{}{}
			\childedgeboth{(\cn)}{($(\cn) + (\hsep,-0.8cm)$)}{}{}
		}
		
		
		
		% ==============  text headers =======================
		\node[draw=none, above=1cm of s3_a_ca] (level_3_current) {current beams};
		\node[draw=none] (level_2_next) at ($(level_3_current) + (-\hsep,0)$) {extended beams};
		\node[draw=none] (level_2_current) at ($(level_2_next) + (-\hsep,0)$) {current beams};
		\node[draw=none] (level_1_next) at ($(level_2_current) + (-\hsep,0)$) {extended beams};
		\node[draw=none] (level_1_current) at ($(level_1_next) + (-\hsep,0)$) {current beams};
		
		\node[draw=none] (level_0_next) at ($(level_1_current) + (-\hsep,0)$) {extend by first $k$-mer};
		\node[draw=none] (level_0_current) at ($(level_0_next) + (-\hsep,0)$) {initial empty beams};
		
		
		% merge text
		\node[draw=none, align=center] at ($($(s2_a_ca_ext)!0.5!(s2_a_ac_dwell)$)!0.5!(s3_a_ac)$) {\footnotesize{merge}\\\footnotesize{identical beams}};
				
        \node[draw=none, align=center] at ($($(s2_b_ca_ext)!0.5!(s2_b_ac_dwell)$)!0.5!(s3_b_ac)$) {\footnotesize{merge}\\\footnotesize{identical beams}};
	\end{tikzpicture}
